Multi-goal Audio-visual Navigation using Sound Direction Map

Over the past few years, there has been a great deal of research on navigation tasks in indoor environments using deep reinforcement learning agents. Most of these tasks use only visual information in the form of first-person images to navigate to a single goal. More recently, tasks that simultaneously use visual and auditory information to navigate to the sound source and even navigation tasks with multiple goals instead of one have been proposed. However, there has been no proposal for a generalized navigation task combining these two types of tasks and using both visual and auditory information in a situation where multiple sound sources are goals. In this paper, we propose a new framework for this generalized task: multi-goal audio-visual navigation. We first define the task in detail, and then we investigate the difficulty of the multi-goal audio-visual navigation task relative to the current navigation tasks by conducting experiments in various situations. The research shows that multi-goal audio-visual navigation has the difficulty of the implicit need to separate the sources of sound. Next, to mitigate the difficulties in this new task, we propose a method named sound direction map (SDM), which dynamically localizes multiple sound sources in a learning-based manner while making use of past memories. Experimental results show that the use of SDM significantly improves the performance of multiple baseline methods, regardless of the number of goals.

==> tex_japanese/abstract.tex <==
\begin{abstract}

近年、深層強化学習エージェントによる室内環境のナビゲーションタスクについて、盛んに研究が行われている。
これらの多くは、一人称視点の画像という視覚の情報のみを用いて、ある一つのゴールまでナビゲーションを行うものである。
しかし近年では、音源をゴールとして聴覚の情報も同時に用いるナビゲーションタスクや、ゴールを一つではなく複数にしたナビゲーションタスクまでも提案されている。
一方で、これらを組み合わせて一般化した、複数の音源がゴールとなっている状況下で、視覚と聴覚の二つの情報を用いるナビゲーションタスクは提案されていない。
そこで、本論文ではこの一般化したタスクであるマルチゴール視聴覚ナビゲーションというフレームワークを提案する。
本研究では、まず、マルチゴール視聴覚ナビゲーションタスクの詳細な定義を行った。
次に、様々な異なる状況下で実験を行うことで、従来のタスクに対するマルチゴール視聴覚ナビゲーションタスクの難しさについて調査した。
調査の結果、マルチゴール視聴覚ナビゲーションには暗に音源を分離しなくてはいけないという難しさがあることがわかった。
そこで、本研究ではこのタスクにおける記憶の重要性に着目し、記憶を用いながら動的に複数の音源について定位を行う手法、Sound Direction Map (SDM)を提案した。
実験により、SDMの活用はゴールの数によらずに複数のベースライン手法に対して精度を向上させることを示した。

\end{abstract}



==> tex_japanese/conclusion.tex <==
\section{CONCLUSION}
\label{conclusion}

本論文では、まず、複数の音源がゴールとなるマルチゴール視聴覚ナビゲーションを提案し、ゴール数が増加することによるナビゲーションへの影響を調査した。
調査の結果、ゴール数が増加することで、極端に性能が劣化する傾向があることがわかった。
それに続く難点調査では、マルチゴール視聴覚ナビゲーションにおける音源分離の重要性が示され、さらに記憶を有効に活用することの重要性も示唆された。

次に、マルチゴール視聴覚ナビゲーションをより高精度に解くための手法、Sound Direction Map (SDM)を提案した。
SDMは、記憶を活かし、動的に複数の音源について定位を行う手法である。
実験により、SDMは全てのゴール数で、全てのベースラインで有用であることが示された。


==> tex_japanese/experiments.tex <==
\section{Experiments}

\subsection{Implementation Details}

\subsubsection{シミュレーション}
エージェントの学習およびテストは、SoundSpaces~\cite{chen2020soundspaces, chen2022soundspaces}というシミュレーター上で、Replica~\cite{straub2019replica}というシーンデータセットを用いて行った。
本研究で用いたSoundSpaces 2.0~\cite{chen2022soundspaces}は、視覚レンダリングを行うシミュレーターHabitat-Sim~\cite{savva2019habitat}に、音響伝搬エンジンRLR-Audio-Propagationを統合することで、Habitat-Simを拡張したシミュレーターである。
また、Replicaは18種類のアパート・オフィス・部屋・ホテルのシーンで構成されるシーンデータセットである。

学習・評価・テスト用のシーンは先行研究\cite{chen2020soundspaces}と同じように分けている。
したがって、テスト時には学習時には用いていないシーンを用いている。
また、今回は評価用のデータセットは用いておらず、一番最後のパラメータ更新によって得られたパラメータによってテストを行なった。
ここで、テストの試行回数は全ての実験において1,000である。



\subsubsection{エピソード生成}

本研究では、簡単すぎるエピソードと難しすぎるエピソードを排除するために、$\boldsymbol{p}_s, \theta_s, \boldsymbol{p}_{g_1}, ..., \boldsymbol{p}_{g_n}$の生成時にいくつか制約をかけている。

まず、簡単すぎるエピソードを排除するために、各地点間の距離は$1\ \mathrm{m}$以上離れるようにし、かつ測地線距離に対するユークリッド距離の比率が1.1より大きくなるようにした。
二つ目の制約の理由は、ほとんど直線のみでゴールに到達できる場合を排除するためである。
ただし、room 2とoffice 1はこれらの制約を満たすことが難しかったため、各地点間の距離は$0.6\ \mathrm{m}$以上離れ、かつ測地線距離に対するユークリッド距離の比率が1.001より大きくなれば良いことにした。

また、簡単すぎるエピソードを排除するために、各地点間の高さは$0.3\ \mathrm{m}$未満になるようにし、かつapartment 0において各地点間の距離が長くなりにくくなるようにした。
具体的には、二点間の距離が$10\ \mathrm{m}$以上なら確率$1.0$、$6\ \mathrm{m}$以上なら確率$0.7$、$5\ \mathrm{m}$以上なら確率$0.6$、$4\ \mathrm{m}$以上なら確率$0.5$、$3\ \mathrm{m}$以上なら確率$0.4$、$3\ \mathrm{m}$未満なら確率$0$で、却下されるというものである。
この制約の理由は、この制約をかけなければapartment 0における性能だけが著しく低くなり、学習曲線が不安定になることがわかったためである。
この問題の本質的な解決には、カリキュラムラーニングの導入が必要であると考えている。


\subsubsection{音源}
特に断りのない限り、先行研究\cite{chen2020soundspaces}にならって、ゴールの音源は訓練には73種類、テストには18種類用いている。
ここで、訓練とテストに重複するような音源はない。
したがって、テストでは訓練時には聞いたことのない音に対する汎化性能を評価していることになる。

各音源は全て、サンプリング周波数44,100$\ \mathrm{Hz}$でサンプリングされた$1$秒分の音データである。
特に断りのない限り、各エピソードでは、音データは$0$秒から$1$秒の間のランダムな時間から再生が開始されるようにしている。

\subsection{ゴール数による比較}

まず、ベースラインとなる手法で、ゴール数のみを変えて実験を行った。
この実験の目的は、ゴール数による難易度の違いを調査することである。
ゴール数$n$は、$n=1,2,3$の三通りで行った。
テスト結果は、表\ref{tab:n_goal_results}のとおりである。


\begin{table}[tb]
    \setlength{\tabcolsep}{4pt}
    \centering
    \caption{
        ゴール数による比較。
        $n$はゴール数を表している。
        ここで、ゴール数が$n$であるとは、訓練とテストの全てのエピソードにおいて、ゴールが$n$個存在しているということを表している
    }
    \label{tab:n_goal_results}
    \begin{tabular}{@{}cccccc@{}}
    \toprule
        手法 & $n$ & $SUCCESS$ & $SPL$ & $PROGRESS$ & $PPL$  \\ \midrule
        ランダム & 1 & \textbf{0.432} & \textbf{0.141} & \textbf{0.432} & \textbf{0.141} \\
        & 2 & 0.167 & 0.048 & 0.377 & 0.070 \\
        & 3 & 0.053 & 0.017 & 0.317 & 0.055 \\ \midrule
        AV-Nav~\cite{chen2020soundspaces} & 1 & \textbf{0.503} & \textbf{0.323} & \textbf{0.503} & \textbf{0.323} \\
        & 2 & 0.179 & 0.119 & 0.229 & 0.142 \\
        & 3 & 0.107 & 0.071 & 0.292 & 0.160 \\ \midrule
        SAVi~\cite{chen2021semantic} & 1 & \textbf{0.647} & \textbf{0.336} & \textbf{0.647} & \textbf{0.336} \\
        & 2 & 0.032 & 0.022 & 0.184 & 0.108 \\
        & 3 & 0.013 & 0.010 & 0.162 & 0.108 \\ \bottomrule
        \end{tabular}
\end{table}


ゴール数を増加させることで、精度が極端に下がる傾向があることがわかった。
$SUCCESS$が大きく下がるのは二つの理由があると考えている。
一つ目の理由は$SUCCESS$は指数関数的に劣化するためである。
これは、スタートから一つのゴールまでに到達する確率が$p$だとすれば、$n$個のゴールに到達できる確率は$p^n$になるからである。
二つ目の理由は、音源分離の必要性が出てくるからであると考えているが、より詳細な議論は次節で行う。
また、$PROGRESS$が下がるのは、エピソードの終了条件が原因であると考えている。
今回の設定では、途中のゴールで失敗してしまえば、そのエピソードは終了する。
したがって、ゴールが複数残っている場合、一つのゴールの失敗は複数のゴールの失敗となる。
これにより、ゴールへの到達率が下がり、$PROGRESS$が下がったと考えられる。


\subsection{複数の音源ゴールがある場合の難点調査}


\subsubsection{大きい音と小さい音}
  

音の大きさによって、つまり音量によって難易度が変化するのかを調査した。
ここでは、小さい音と大きい音へ到達率の違いを比較している。
ただし、これらの音は全て訓練では用いていない音から選択されている。
また、小さい音の集合の音の鳴る長さの平均と大きい音の集合の音の鳴る長さの平均は近くなるように、これらの音は選択されている。

\begin{table}[tb]
    \caption{
        小さい音(top)と大きい音(bottom)への到達率の比較。
        $n$-smallとは、小さい音の集合から$n$個選択されたものがゴールになることを表す。
        また、$n$-bigとは大きい音の集合から$n$個選択されたものがゴールになることを表す。
        ただし、学習時には訓練用の73種類全ての音源を用いている。
    }
    \label{tab:big_and_small}
    \centering
    %% \begin{tabular}{@{}ccc@{}}
    %% \toprule
    %%     & ゴール形式 & 到達率 \\ \midrule
    %%     小さい音 & 1-small & 0.441 \\
    %%     & 2-small & 0.232 \\
    %%     & 1-small-1-big & 0.187 \\ \midrule
    %%     大きい音 & 1-big & 0.449 \\
    %%     & 2-big & 0.209 \\
    %%     & 1-smal-1-big & 0.253 \\ \bottomrule
    %% \end{tabular}
    \begin{tabular}{@{}ccccccc@{}}
      \toprule
      & \multicolumn{2}{c}{1-goal task} & \multicolumn{3}{c}{2-goal task} \\
      \cmidrule(lr){2-3} \cmidrule(lr){4-6} 
      & 1-small & 1-big & 2-small & 2-big & 1-small-1-big \\
      \midrule
      small & 0.441 & N/A & 0.232 & N/A & 0.187 \\
      big & N/A & 0.449 & N/A & 0.209 & 0.253 \\
      \bottomrule
    \end{tabular}
\end{table}

表\ref{tab:big_and_small}はその結果である。
この結果から、大きい音も小さい音も、同時に大きい音が鳴ると精度が下がることがわかった。
これは、大きい音は遠くにいても聞こえるため、ノイズになりやすいからであると考えている。


\subsubsection{長い音と短い音}

音の鳴る時間の長さによって、難易度が変化するのかを調査した。
ここでは、短い音と長い音へ到達率の違いを比較している。
ただし、これらの音は全て訓練では用いていない音から選択されている。
また、短い音の集合の最大音量の平均と、長い音の集合の最大音量の平均は近くなるようにこれらの音は選択されている。

\begin{table}[tb]
    \centering
    \caption[短い音と長い音への到達率]
    {
        短い音(top)と長い音(bottom)への到達率の比較。
        $n$-shortとは、短い音の集合から$n$個選択されたものがゴールになることを表す。
        また、$n$-longとは長い音の集合から$n$個選択されたものがゴールになることを表す。
        ただし、学習時には訓練用の73種類全ての音源を用いている。
    }
    \label{tab:long_and_short}
    %% \begin{tabular}{@{}ccc@{}}
    %% \toprule
    %%     & ゴール形式 & 到達率 \\ \midrule
    %%     短い音 & 1-short & 0.235 \\
    %%     & 2-short & 0.160 \\
    %%     & 1-short-1-long & 0.141 \\ \midrule
    %%     長い音 & 1-long & 0.632 \\
    %%     & 2-long & 0.255 \\
    %%     & 1-short-1-long & 0.262 \\ \bottomrule
    %% \end{tabular}
    \begin{tabular}{@{}ccccccc@{}}
      \toprule
      & \multicolumn{2}{c}{1-goal task} & \multicolumn{3}{c}{2-goal task} \\
      \cmidrule(lr){2-3} \cmidrule(lr){4-6} 
      & 1-short & 1-long & 2-short & 2-long & 1-short-1-long \\
      \midrule
      short & 0.235 & N/A & 0.160 & N/A & 0.141 \\
      long & N/A & 0.632 & N/A & 0.255 & 0.262 \\
      \bottomrule
    \end{tabular}
\end{table}

表\ref{tab:long_and_short}はその結果である。
この結果から、長い音も短い音も、同時に長い音が鳴ると精度が下がることがわかった。
これは、長い音は常になり続けているため、もう一方の音のノイズになりやすいからであると考えている。



\subsubsection{同一音と不同音}

複数の音源がゴールとなる場合に、それらの音の種類が同じであるのか、それとも異なるのかによって、難易度が変化するのかを調査した。
ここでは、学習時には重複も許してランダムに二つの種類の音源を用いており、テスト時には、同じ二つの種類・異なる二つの種類・重複も許してランダムに二つの種類を用いる三つの状況で行った。
結果は表\ref{tab:same_and_different_sound}のようになった。

\begin{table}[tb]
    \centering
    \caption{
        同じ二つの音が鳴る場合と異なる二つの音が鳴る場合の比較。
        ゴールは二つあり、手法はAV-Nav\cite{chen2020soundspaces}である。
    }
    \label{tab:same_and_different_sound}
    \begin{tabular}{@{}ccccc@{}}
    \toprule
        & $SUCCESS$ & $SPL$ & $PROGRESS$ & $PPL$  \\ \midrule
        同じ音 & \textbf{0.193} & \textbf{0.131} & \textbf{0.244} & \textbf{0.155} \\
        異なる音 & 0.181 & 0.120 & 0.232 & 0.145 \\
        ランダム & 0.179 & 0.119 & 0.229 & 0.142 \\ \bottomrule
        \end{tabular}
\end{table}

異なる音が鳴っている方が、精度が低くなることがわかった。
これは、大きい音と小さい音が鳴っているときは小さい音への、長い音と短い音が鳴っているときは短い音への到達率が下がっているように、異なる性質の音が鳴ることで、一方の音への到達率が下がるからではないかと考えている。
異なっているときは一方がかき消されることが多くなり、到達率が下がるのではないかと考えている。
これらの結果は、音源分離の重要性を示している。




\subsubsection{鳴るタイミング}

複数の音の鳴るタイミングによって、難しさが変化するのかを調査した。
結果は、表\ref{tab:sound_timing}のようになった。

\begin{table}[tb]
    \centering
    \caption{
        二つの音が鳴るタイミングによる比較。
        ゴールは二つあり、手法はAV-Nav\cite{chen2020soundspaces}である。
        この実験では、音源は電話の音のみが用いられている。
        また、学習はランダムの設定で行なっている。
    }
    \label{tab:sound_timing}
    \begin{tabular}{@{}ccccc@{}}
    \toprule
        & $SUCCESS$ & $SPL$ & $PROGRESS$ & $PPL$ \\ \midrule
        重なる & \textbf{0.792} & \textbf{0.430} & \textbf{0.868} & \textbf{0.444} \\
        重ならない & 0.735 & 0.410 & 0.811 & 0.424 \\
        ランダム & 0.736 & 0.413 & 0.820 & 0.440 \\ \bottomrule
    \end{tabular}
\end{table}

同じ音が二つ鳴っている場合、音に重複がない方が精度が低くなるという結果を得た。
これは、交互に同じ音が鳴ると音源の定位が難しくなるからであると考えている。
エージェントには音源の数は与えられていないため、同じ音が交互に別の場所で鳴ると、一つの音が行き来していると判断してしまう可能性がある。
このことから、動的複数音源定位の履歴を表現する手法が重要であると考えられる。



\subsection{Sound Direction Map}

\subsubsection{定量評価}

SDMの有用性を示すために、ベースラインにおいてSDMを用いた場合と用いなかった場合の性能を比較した。
表\ref{tab:dm_results}はその結果である。

\begin{table}[tb]
    \setlength{\tabcolsep}{3pt}
    \centering
    \caption{
        SDMの定量評価。
        $n$はゴール数を表す。
    }
    \label{tab:dm_results}
    \begin{tabular}{@{}llcccc@{}}
    \toprule
        $n$~ & 手法 & $SUCCESS$ & $SPL$ & $PROGRESS$ & $PPL$ \\ \midrule
        1 & AV-Nav~\cite{chen2020soundspaces} & 0.503 & 0.323 & 0.503 & 0.323  \\
        & SAVi~\cite{chen2021semantic} & 0.647 & 0.336 & 0.647 & 0.336 \\
        & AV-Nav~\cite{chen2020soundspaces} w/ SDM & 0.610 & 0.354 & 0.610 & 0.354 \\
        & SAVi~\cite{chen2021semantic} w/ SDM & \textbf{0.874} & \textbf{0.574} & \textbf{0.874} & \textbf{0.574} \\ \midrule
        2 & AV-Nav~\cite{chen2020soundspaces} & 0.179 & 0.119 & 0.229 & 0.142  \\
        & SAVi~\cite{chen2021semantic} & 0.032 & 0.022 & 0.184 & 0.108 \\
        & AV-Nav~\cite{chen2020soundspaces} w/ SDM & \textbf{0.332} & \textbf{0.172} & \textbf{0.506} & \textbf{0.232} \\
        & SAVi~\cite{chen2021semantic} w/ SDM & 0.183 & 0.109 & 0.400 & 0.206 \\ \midrule
        3 & AV-Nav~\cite{chen2020soundspaces} & 0.107 & 0.071 & 0.292 & 0.160 \\
        & SAVi~\cite{chen2021semantic} & 0.013 & 0.010 & 0.162 & 0.108 \\
        & AV-Nav~\cite{chen2020soundspaces} w/ SDM & 0.174 & 0.101 & 0.368 & 0.186 \\
        & SAVi~\cite{chen2021semantic} w/ SDM & \textbf{0.335} & \textbf{0.221} & \textbf{0.571} & \textbf{0.336} \\ \bottomrule
    \end{tabular}
\end{table}

全てのゴール数と全てのベースラインにおいて、SDMを用いることで性能を向上させることができた。
さらに、SDMはゴール数増加による劣化を抑える傾向があることもわかった。
このような結果を得た理由は、記憶を有効に活用し、複数の音源についての定位がより正確にできるようになったからであると考えている。

\subsubsection{定性評価}

\begin{figure*}[t]
    \begin{center}
        \centering
        \includegraphics[scale=0.7]{fig/2g-nav-traj.pdf}
        \caption{
            ナビゲーションの軌跡比較。
            上段がAV-Nav w/o SDMで、下段がAV-Nav w/ SDMである。
            また、Pathの色はステップの経過を表している。
            ステップが経過するにつれ、青から赤へ変化する。
        }
        \label{fig:qualitative_eval}
    \end{center}
\end{figure*}


図\ref{fig:qualitative_eval}はSDMを用いた場合と用いなかった場合の、エージェントの軌跡の比較である。
SDMを用いることで無駄な行動が減っていることがわかる。
これは、音源定位がより正確にできるようになったからではないかと考えている。
また、AV-Nav w/o SDMの失敗例では、長く彷徨っている例が見られた。
これは、音源定位が正確にできず、どこにゴールがあるかを判断できずにいるからではないかと考えている。
また、w/ SDMでは、障害物に引っかかり、失敗してしまうケースが見られた。
これは、SDMにより、障害物の反対側に音源があると判断されてしまっているからであると考えている。



==> tex_japanese/introduction.tex <==
\section{INTRODUCTION}

深層強化学習エージェントによる室内環境の視覚ナビゲーションタスクはここ10年で特に注目されている研究分野である。
ベーシックな視覚ナビゲーションは、一人称視点の画像という視覚情報のみを用いて、ある一つのゴールまでナビゲーションを行うものである。
近年では、より発展的なタスクが生まれており、視覚だけでなく聴覚の情報も同時に用いて音源へナビゲーションを行うAudio-Visual Navigation~\cite{chen2020soundspaces}や、一つではなく複数のゴールへナビゲーションを行うMulti-Object Navigation (MultiON)~\cite{wani2020multion}とよばれるタスクも提案されている。
一方、視覚の情報と聴覚の情報の二つを用いて、複数の音源ゴールへナビゲーションを行うタスク、すなわち、先に挙げた視聴覚ナビゲーションとマルチオブジェクトナビゲーションを組み合わせたようなタスクはいまだに提案されていない。
実応用を考えると、人命救助や鳥獣害駆除といった、聴覚情報が有効で、かつ必ずしもゴールが一つとは限らないようなタスクは多く存在する。
%むしろこれらのタスクでは、複数のゴールがあると考えるのが自然である。

\begin{figure}[t]
    \begin{center}
        \centering
        \includegraphics[width=\linewidth]{fig/multi-goal-audio-visual-navigation.pdf}
        \caption{
            マルチゴール視聴覚ナビゲーションの様子。
            ここでは、室内環境において三つの異なる音源へナビゲーションを行っている。
            エージェントは、一人称視点の視覚の情報と三つの異なる音源の音が重なった聴覚の情報を観測し、適切な行動選択を行わなければならない。
        }
        \label{fig:multi_goal_av_nav}
    \end{center}
\end{figure}

%したがって、こうした応用先を念頭におき、視覚の情報と聴覚の情報の二つを用いた複数の音源ゴールへのナビゲーションタスクについて研究することは、意義があると考えられる。視聴覚ナビゲーションだけでは、ある一つのゴールに到達するまでに得た有効な情報を捨ててしまうことになる。マルチオブジェクトナビゲーションだけでは、聴覚情報という有効な情報を捨ててしまうことになる。しかし、効率的なナビゲーションを行えるようにするためには、可能な限り、得ることのできる有効な情報は捨てずにあつかうべきである。
本研究では、視聴覚ナビゲーションとマルチオブジェクトナビゲーションを組み合わせた新しいタスクであるMulti-Goal Audio-Visual Navigationを提案する（図\ref{fig:multi_goal_av_nav}）。
マルチゴール視聴覚ナビゲーションを解くためには、三つの重要な要素がある。
それは、音源分離・記憶・行動計画である。
まず、強化学習エージェントは、複数の音が重なった音を観測する。
そのため、正確な音源分離は、各音源に対する音源定位の精度向上に重要な役割を果たす。
また、ある一つのゴールへ到達するまでに取得した情報を記憶しておくことで、次のゴールへ効率的にナビゲーションを行えるようになることが期待できる。
さらに、そもそもどの音源を次のゴールにすると効率的な経路計画となるのかを推論しなくてはいけないという点において、行動計画は重要である。

本研究には、二つの目的がある。
第一の目的は、マルチゴール視聴覚ナビゲーションの難しさがどこにあるのかを明らかにすることである。
先にも述べたが、複数の音源ゴールがある場合の視聴覚ナビゲーションに対する先行研究はない。
本研究では、多様な状況下でマルチゴール視聴覚ナビゲーションを行うことで、どこに難しさがあるのかを明らかにする。
第二の目的は、マルチゴール視聴覚ナビゲーションをより高精度に解くための手法を提案することである。
本研究では、先述の三つの課題を解決するために、implicitな動的複数音源定位に基づく手法Sound Direction Map (SDM)を提案する。
SDMは、複数の音源を同時に定位することで経路計画を助ける。
また、SDMは記憶を有効に活用することで動的に更新される。
この動的な更新手法により、過去の音源定位情報を活用することで音源分離の性能を向上させ、その結果、音源定位の性能をさらに高める可能性がある。

本論文の主な貢献は以下の三つである。

\begin{itemize}[leftmargin=*]
\item 新しいナビゲーションフレームワークであるマルチゴール視聴覚ナビゲーションを提案し、様々な状況下でテストすることで、このタスクの難しさがどこにあるのかを検証した。
\item マルチゴール視聴覚ナビゲーションを効率的に解く手法として、implicitな動的複数音源定位の履歴を表現するSound Direction Map (SDM)を提案した。
\item SoundSpaces 2.0において、提案するSDMを用いることで、複数のベースライン手法に対する精度向上を示した。
\end{itemize}

==> tex_japanese/method.tex <==
\section{METHODS}

\begin{figure}[t]
    \begin{center}
        \centering
        \includegraphics[scale=0.3]{fig/direct_map.pdf}
        \caption{
            Sound Direction Map (SDM)の概要。
            エージェントを囲う黒い円によってSDMが表現されている。
            ここでは、二つの音源がある場合の例を示している。
            エージェントから見て音源方向のSDMのノードの値が高くなる様子が、ノードの色の濃さで表現されている。
        }
        \label{fig:direct_map_abst}
    \end{center}
\end{figure}

\begin{figure*}[t]
    \begin{center}
        \centering
        \includegraphics[scale=0.6]{fig/direct-map-encoder.pdf}
        \caption{
            AV-Nav\cite{chen2020soundspaces}のネットワークアーキテクチャーにSDM作成のためのネットワークを適用した様子。
            Sound Direction Map Encoderが、今回提案するSDM作成のためのネットワークアーキテクチャである。
            ここで、$\boldsymbol{a}_{t}$と$\hat{\boldsymbol{d}}_t$は、それぞれ時刻$t$における、行動を表すワンホットベクトルとSDMの予測を表す。
            入力には、音の観測$A_t$だけではなく、前回の行動を表すワンホットベクトル$\boldsymbol{a}_{t-1}$と前回のSDMの予測$\hat{\boldsymbol{d}}_{t-1}$の二つも入力している。
        }
        \label{fig:direct_map_encoder}
    \end{center}
\end{figure*}

\subsection{Baselines}

本研究ではベースライン手法として、最もシンプルなランダム行動選択方法に加え、二つのよく知られた深層強化学習手法をテストする。
それぞれの手法について、下記に詳しく説明する。

\subsubsection{Random}
このエージェントは、$\{MoveForward, TurnLeft, TurnRight\}$の三つの中から、ランダムに行動を選択する。
ただし、ゴールである音源の半径$1\ \mathrm{m}$未満にエージェントがいる場合は$Found$を必ず選択する。

\subsubsection{AV-Nav \cite{chen2020soundspaces}}
エンドツーエンドの深層強化学習手法。
一人称視点の画像とスペクトログラムを入力とする、GRUをベースとした方策ネットワークを持つ。
これは、視聴覚ナビゲーションタスクで一番はじめに提案された手法であり、最もシンプルな手法である。

\subsubsection{SAVi \cite{chen2021semantic}}
Transformerをベースとした方策ネットワークを持つ深層強化学習手法。
一人称視点の画像とスペクトログラムに加え、エージェントの姿勢と前回の行動を入力とする。
さらに、ゴールとなる音源のカテゴリとその位置を予測するGoal Descriptor Networkを持ち、カテゴリの予測部分は事前学習される。
また、ポリシーの学習は2段階に分かれる。
first stageでは、Transformerのメモリーサイズを1にしてObservationの埋め込みを学習する。
second stageでは、Observationの埋め込みの学習をfreezeさせてメモリーサイズを150にしてその他の場所を学習させる。

本研究の対象タスクはSemantic Audio-Visual Navigation~\cite{chen2021semantic}ではないことと、マルチゴールへの拡張の困難さのため、本研究ではGoal Descriptor Networkは使っていない。


\subsection{Proposed Method}


以下では、記憶を用いて明示的かつ動的に複数の音源の定位を行うことを可能にする提案手法、Sound Direction Map (SDM)について説明する。

SDMとは、エージェントを中心として、どの方向のどれくらい離れた場所に音源があるのかを表すものである。
図\ref{fig:direct_map_abst}では、エージェントを囲う黒いノードでSDMが表現されている。
SDMでは、エージェントから音源までの距離が近ければ近いほど、その音源の方向にあるノードの値が高くなる。
こうすることで、SDMは、複数の音源に対して方向と距離による音源定位を可能にする。
ただし、同じ方向に複数音源がある場合は最も近い音源だけが考慮される。

各ノードの値は、その方向にある音源までのGeodesic Distanceの逆数としている。
ここで、ユークリッド距離ではなく測地線距離を用いた理由は、音波は壁などの障害物によって反射・回折・減衰を起こすため、測地線距離の方が予測がしやすいと考えたからである。
また、今回は距離が$1\ \mathrm{m}$以内の音源に対しては、クリッピングを行っている。
これには二つの理由がある。一つは、エージェントは半径$1\ \mathrm{m}$以内であれば厳密に定位を行う必要がないためである。
もう一つは、SDMを作成するエンコーダーの学習時に、非常に大きな値に過剰に反応してしまうことを防ぐためである。

本研究では、ニューラルネットワークを用いることで、エージェントが行動を繰り返しながら、動的にSDMを予測していく手法を提案する。
今回提案するニューラルネットワークのアーキテクチャーは図\ref{fig:direct_map_encoder}のとおりである。

今回、AV-Nav\cite{chen2020soundspaces}とSAVi\cite{chen2021semantic}のネットワークにSDMを適用させ、エンドツーエンドで学習させた。
SAViでは、Observation Encoderの一部としてSound Direction Map Encoderを追加する。
つまり、SAViでは、Sound Direction Map Encoderはfirst stageでのみ学習させる。
SDMを作成するネットワークの重みの更新には、方策ネットワークから流れてくる勾配に加え、予測したSDMと真のSDMの平均二乗誤差（Mean Squared Error; MSE）による勾配も用いている。

また、学習時には、前回のSDMとして、前回のSDMの真値$\boldsymbol{d}_{t-1}$を入力している。
我々は予備実験において、前回のSDMとして、前回の自身の予測$\hat{\boldsymbol{d}}_{t-1}$を入力して学習させる場合もテストした。
実験により、予測値よりも真値を入力して学習させる方が性能が高くなることが分かったため、その方法を採用した。
ただし、テスト時とSAViの学習のsecond stageでは真値を使用せず、前回の自身のSDM予測値を入力している。

さらに、学習時にはDropoutという工夫を行った。
これは、前回のSDMとして入力するSDMの各ノードの値を、ある一定の確率で0にするというものである。
これは、現在のSDMを予測するときに、前回のSDMに依存しすぎることを防ぐことを目的としている。
なぜなら、前回のSDMとして入力される$\hat{\boldsymbol{d}}_{t-1}$が、真の前回のSDM $\boldsymbol{d}_{t-1}$を適切に予測しているとは限らないためである。
ただし、SAViの学習のsecond stageではDropoutは行わない。


\subsection{Reward}

時刻$t$にエージェントが受け取る報酬は以下のように定義した。
\[
r_t = r_{\mathrm{found}} - \Delta_{\mathrm{geo}} - 0.01 \label{eq:reward_definition}
\]
ここで、$r_{\mathrm{found}}$は、エージェントが時刻$t$においてゴールに到達した場合$5$になり、到達していない場合は$0$になる。
また、$\Delta_{\mathrm{geo}} \in \mathbb{R}$は、まだ到達していないすべてのゴールに到達するための最小の測地線距離の変化量である。
つまり、$\Delta_{\mathrm{geo}}$は、まだ到達していないすべてのゴールに到達するための最小測地線距離が、小さくなれば負の値になり、大きくなれば正の値になる。



\subsection{Training}

エージェントの学習にはDecentralized Distributed Proximal Policy Optimization（DD-PPO）\cite{wijmans2019dd}とよばれる、分散深層強化学習手法を用いた。
AV-Navを用いた学習には4 GPUsを利用し各GPUに四体のワーカーを配置させた。
また、SAViを用いた学習には16 GPUsを利用し各GPUに二体のワーカーを配置させた。

本研究におけるハイパーパラメータの設定は以下のとおりである。
まず、SDMのユニット数は$8$にし、各ユニットでドロップアウトが実行される確率は$0.2$にした。
さらに、SDMを予測するネットワークの重み更新時の勾配において、予測したSDMと真のSDMの平均二乗誤差による勾配の係数は、$100$にしている。
また、AV-NavとSAViに関するハイパーパラメーターは、SoundSpacesのデフォルトのパラメータを用いた。
ただし、重みの更新回数はAV-Navでは1,250回であり、SAViではfirst stageは570回、second stageは580回である。





==> tex_japanese/related.tex <==
\section{RELATED WORK}

\subsection{Sound Source Localization}

Sound Source Localization (SSL) とは、観測した音のデータから、その音の音源の位置を推定することである\cite{rascon2017localization}。
近年では、この音源定位を深層学習を用いて行う手法が数多く提案されている\cite{grumiaux2022survey}。
これらの中には、Maら\cite{ma2015exploiting}やHeら\cite{he2018deep}といった、本研究と同じで複数の音源を定位する問題を解いているものもある。
これらでは、Multilayer Perceptron (MLP)やConvolutional Neural Network (CNN)をベースとして複数の音源の到来方向を推定する手法が提案された。
さらに、Adavanneら\cite{adavanne2019localization}では、Convolutional Recurrent Neural Network (CRNN)を用いることで、音源が動いている状況下で複数の音源の到来方向を追跡する手法が提案されている。

本論文でも、深層学習を用いることで音源定位を行う手法を提案する。
特に、定位するべき音源が複数がある状況で、強化学習手法によって観測者が動きながら、動的に音源定位を行う手法を提案する。


\subsection{Visual Navigation}

Visual Navigationとは、ある環境に置かれた自律移動ロボットが、視覚の情報を用いることで、スタートからゴールまで適切かつ安全な経路を生成するプロセスのことである\cite{bonin2008visual}。
本研究で扱う三次元の室内環境における視覚ナビゲーションでは、視覚の情報として、一人称視点のRGBD画像が用いられることが多い。
視覚ナビゲーションでは、このような視覚の情報を利用することで環境を理解しながら、自己位置や目標位置を推定し、適切な行動選択を行うことが要求される。

視覚ナビゲーションを解くための手法は数多く提案されており、近年ではそのほとんどが深層強化学習をベースとしたものになっている。
Parisottoら\cite{DBLP:journals/corr/ParisottoS17}は、ナビゲーションの部分観測性には記憶が重要であるということに着目し、適応的に環境の空間的構造を記憶するための二次元マップを作成する手法Neural Mapを提案した。
また、Chaplotら\cite{chaplot2019learning, chaplot2020object}は、マップの作成と同時に自己の姿勢推定も行う手法を提案した。
これらは明示的にマップを作成する手法である一方で、明示的にマップを作成しない手法も存在する。
Fangら\cite{fang2019scene}やFukushimaら\cite{9812027}は、観測の埋め込みを履歴として保存し、Transformer~\cite{vaswani2017attention}を用いることで長期的な記憶の考慮を可能にした手法を提案した。
また、RGB画像の深度予測や閉ループ検出などのナビゲーションと直接は関係しない補助タスクを同時に解くことで、ナビゲーションの性能を高めようとする手法も提案されている\cite{mirowski2017learning, 9370169}。

本研究に最も近い視覚ナビゲーションの先行研究は、Waniら\cite{wani2020multion}である。
Waniら\cite{wani2020multion}では、Multi-Object Navigation (MultiON) というタスクが提案された。
MultiONでは、指定された複数の物体に、指定された順番でナビゲーションを行わなければならない。
したがって、複数のゴールへナビゲーションを行わなければならないという意味で、本研究に近いタスクであるといえる。
ただし、MultiONと違い、本研究で扱うマルチゴール視聴覚ナビゲーションではゴールに到達するべき順番は決められていない。
よって、どのゴールから向かうべきかをエージェント自身が考えなければならない。


\subsection{Audio-Visual Navigation}

Audio-Visual Navigationとは、視覚だけではなく、聴覚の情報も用いて、音源までナビゲーションを行うものである。
聴覚の情報は、ナビゲーションタスクに重要な自己位置と目標位置の推定や、環境の幾何学的構造の理解に役立つ可能性がある。
実際、Chenら\cite{chen2020soundspaces}は実験的に、ナビゲーションで聴覚の情報を用いることの有用性を示している。

近年では、この視聴覚ナビゲーションについて盛んに研究が行われており、多様なタスクが提案されてきている。
Majumder and Pandey~\cite{majumdersemantic}では、妨害音として目標以外の音源を用いる視聴覚ナビゲーションが提案された。
また、従来の視聴覚ナビゲーションでは音が鳴り止まないことが仮定されていたが、Chenら\cite{chen2021semantic}では、エピソード開始直後の短時間しか音が鳴らない視聴覚ナビゲーションが提案された。
さらに、音源が動くといったもの\cite{younes2021catch, yu2021sound}や、落ちた物体を探すというかなり現実的なもの\cite{gan2022finding}までも提案されてきている。

また、視聴覚ナビゲーションを解く手法もすでにいくつか提案されている。
Chenら\cite{chen2020soundspaces}は、視覚の観測である画像の特徴量と聴覚の観測であるスペクトログラムの特徴量を、Gated Recurrent Unit (GRU)~\cite{chung2014empirical}に入力して方策を得るというシンプルな手法AV-Navを提案した。
ついでChenら\cite{chen2020learning}は、観測した深度画像とスペクトログラムから、環境の地理的なマップとその場所における音の強度を保存するアコースティックマップを作成し、次に到達するべきウェイポイントを生成するという手法AV-WaNを提案した。
そしてChenら\cite{chen2021semantic}は、方策ネットワークをTransformerベースにし、かつ音源のカテゴリと相対位置を予測するモジュールも提案した。
さらに、Tatiyaら\cite{tatiya2022knowledge}は、物体間と物体-領域間の関係を表すKnowledge Graphを活用し、そこからGraph Convolutional Network (GCN)~\cite{kipf2017semisupervised}を用いて特徴量を抽出するという知識ドリブンな手法K-SAVENを提案した。

多様なタスクや手法について研究されている一方で、一つのエピソードで複数の音源へナビゲーションを行うタスクは研究されていない。
したがって、この問題を扱うのは本研究がはじめてである。

また、視聴覚ナビゲーションに関する先行研究では、シミュレータとしてSoundSpaces~\cite{chen2020soundspaces, chen2022soundspaces}がよく用いられる。
SoundSpacesには、1.0~\cite{chen2020soundspaces}と 2.0~\cite{chen2022soundspaces}の二つのバージョンがある。
2.0はより現実的な設定に近づいている。
そのため、本研究では2.0を用いた。




==> tex_japanese/task.tex <==
\section{Multi-Goal Audio-Visual Navigation}

\subsection{Task Definitions}


本論文で提案するMulti-Goal Audio-Visual Navigationとは、一つのエピソードで複数のゴールへナビゲーションを行う視聴覚ナビゲーションである（図\ref{fig:multi_goal_av_nav}）。
したがって、エージェントは複数の音が重なった音を観測し、それぞれの音源に対して定位しなければならない。
また、聴覚の情報を用いること以外の、マルチオブジェクトナビゲーションとの大きな違いとして、各ゴールにナビゲーションを行う順番が指定されていないことが挙げられる。
よって、どのような順番で各音源へナビゲーションを行うと効率的であるのかを、エージェント自身が考えなければならない。
以下では、マルチゴール視聴覚ナビゲーションについてより詳細な説明をする。

形式的には、一つのエピソードは、組$\{E, \bm{p}_s, \theta_s, \bm{p}_{g_1}, ..., \bm{p}_{g_n}, S_{g_1}, ..., S_{g_n}\}$で定義される。
ここで、$E$はエピソードで用いるシーン環境を表し、$\bm{p}_s \in \mathbb{R}^3$と$\theta_s \in [0, 2\pi]$はそれぞれ、エージェントの開始時の位置と向いている方向を表す。
また、$n \in \mathbb{N}$はゴールの数を表しており、各$i \in \{1, ..., n\}$に対し、$\bm{p}_{g_i} \in \mathbb{R}^3$と$S_{g_i} \in SoundCategory$はそれぞれ、ゴール$g_i$の位置と音源のカテゴリを表している。
ここで、$SoundCategory$は音のカテゴリの集合を表し、本研究では合計$91$種類の音のカテゴリを用いている。
以上より、マルチゴール視聴覚ナビゲーションとは、環境$E$において、スタート$(\bm{p}_s, \theta_s)$から出発し、$S_{g_1}, ..., S_{g_n}$の重なった音を聞きながら、ゴール位置$\bm{p}_{g_1}, ..., \bm{p}_{g_n}$を推定し、到達していくことであるということができる。

今回、マルチゴール視聴覚ナビゲーションでは、AudioGoal~\cite{chen2020soundspaces}とよばれるゴール形式を採用している。
AudioGoalとは、ゴールは音源であり、周期的に発生するその音の情報から位置を推測しなければならないというものである。
また、ゴールは視覚的には示されていないため、聴覚の情報のみを頼りにゴール位置を推定する必要がある。

また、エージェントがゴールに到達すると、そのゴールの音源はそれ以降音を発しない。
つまり、エージェントがゴール$g_i$に到達すると、それ以降エージェントは$S_{g_i}$の音を観測しなくなる。
よって、現在エージェントが観測している音は、まだ到達していない音源から発せられていることになる。
したがって、エージェントは現在観測している音が、すでに到達した音源から発せられているものであるのか、ないしはまだ到達していない音源から発せられているものであるのかを判定する必要はない。



\subsection{Action Space}

マルチゴール視聴覚ナビゲーションにおける、エージェントの行動空間は
\[ 
\mathcal{A} = \{MoveForward, TurnLeft, TurnRight, Found\} \label{eq:action_space}
\]
である。
$MoveForward$を選択すると、エージェントは環境を$0.25\ \mathrm{m}$進む。
$TurnLeft$または$TurnRight$を選択すると、それぞれ左または右に$10^\circ$回転する。
また、ゴールである音源の半径$1\ \mathrm{m}$未満で$Found$を選択することができれば、その音源に到達したことを意味する。
以上の具体的な数値は、SoundSpaces 2.0のデフォルトの設定である。

エピソードが終了するのは、以下の三つの条件のうち、いずれかが満たされたときである。
一つ目は、全てのゴールに到達することである。
二つ目は、ゴールから半径1以上離れた場所で$Found$を選択することである。
三つ目は、合計の行動回数が2,500を超えることである。
この行動回数の上限は先行研究\cite{wani2020multion}を参考にして設定した。

\subsection{Observation Space}

マルチゴール視聴覚ナビゲーションでエージェントが観測することができるのは、視覚の情報と聴覚の情報である。
視覚の情報としては、一人称視点の$128 \times 128$のRGBD画像を用いている。
また、聴覚の情報としては、$257 \times 69$のスペクトログラムを用いている。
音の方式は、先行研究に倣って2チャネルのバイノーラル音を用いている。

本研究におけるスペクトログラム作成の手順は、以下のとおりである。
まず、サンプリング周波数44,100$\ \mathrm{Hz}$でサンプリングした$0.25$秒分の離散的な音の時系列のデータを獲得する。
次に、その時系列データに対して短時間フーリエ変換を行い、各時間の各周波数の成分の振幅を求める。
ここで、窓関数（Window Function）はハニング窓（Hanning Window）、フレームサイズは$512$、フレームシフトは$160$である。
最後に、各値に対して$1$を足して対数をとった結果を各成分の強さとして、スペクトログラムを作成する。


\subsection{Metrics}


本研究では、$SUCCESS$、$SPL$、$PROGRESS$、$PPL$の四つの評価指標を用いた。
以下では、これらの詳細を説明する。

$SUCCESS$は、テストしたエピソードの数を$N$とすると、以下で表される。
\[
SUCCESS = \frac{1}{N} \sum_{i = 1}^N S_i
\]
ここで、$S_i \in \{0, 1\}$はエピソード$i \in \{1, ..., N\}$において全てのゴールに到達できたかどうかのバイナリーの値である。
つまり、$i$番目のエピソードにおいて、エージェントが全てのゴールに到達できたら$S_i = 1$であり、一つでも到達できなければ$S_i = 0$となる。

$SPL$は以下で表される\cite{anderson2018evaluation}。
\[
SPL = \frac{1}{N} \sum_{i = 1}^N S_i \frac{l_i}{\max(l^A_i, l_i)}
\]
ここで、$l^A_i \in \mathbb{R}$はエージェントが実際に進んだ経路の長さ、$l_i \in \mathbb{R}$は最短経路の長さを表している。
つまり、たとえエージェントが全てのゴールに到達できても、最短経路に近い経路で進まなければ、$SPL$は高い値にはならない。

$PROGRESS$は以下で表される\cite{wani2020multion}。
\[
PROGRESS = \frac{1}{N} \sum_{i = 1}^N \frac{n^A_i}{n}
\]
ここで、$n \in \mathbb{N}$はゴールの数、$n^A_i \in \mathbb{N}$はエージェントがエピソード$i$で到達したゴールの数を表している。
つまり、$SUCCESS$とは異なり、全てのゴールに到達しなくても、一つのゴールにさえ到達していれば値が$0$になることはない。

$PPL$は以下で表される\cite{wani2020multion}。
\[
PPL = \frac{1}{N} \sum_{i = 1}^N \frac{n^A_i}{n} \frac{l^\mathrm{MG}_i}{\max(l^A_i, l^\mathrm{MG}_i)}
\]
ここで、$l^\mathrm{MG}_i \in \mathbb{R}$は、スタート地点からエージェントが到達した全てのゴール地点を通るための最短経路の長さを表す。
つまり$PPL$は、より多くのゴールへ、より最短経路に近い経路で到達することで値が高くなる。

ただし、Waniら\cite{wani2020multion}では到達するべき順番が決められている一方で、本研究では到達するべき順番が決められていない。
そのため、$l^\mathrm{MG}_i$の計算方法は異なる。
仮に、エピソード$i$においてエージェントが$g_1, ..., g_{n^A_i}$の順でゴールに到達したとし、スタートの位置が$\bm{p}_s$であったとする。
また、点$\bm{p}, \bm{q}$間の最短経路の長さは$d_{\mathrm{min}}(\bm{p}, \bm{q})$で表すことができるとする。
このとき、Waniら\cite{wani2020multion}では$l^\mathrm{MG}_i = d_{\mathrm{min}}(\bm{p}_{s}, \bm{p}_{g_1}) + \sum_{j=2}^{n^A_i} d_{\mathrm{min}}(\bm{p}_{g_{j-1}}, \bm{p}_{g_j})$と表される。
しかし、本研究では到達するべき順番が決められていないため、この計算によって正しく$l^\mathrm{MG}_i$が計算できるとは限らない。
代わりに、以下のようにして計算する必要がある。
\[
l^\mathrm{MG}_i = \min_{\sigma \in T_{n^A_i}} \left\{ d_{\mathrm{min}}(\bm{p}_{s}, \bm{p}_{g_{\sigma(1)}}) +  \sum_{j=2}^{n^A_i} d_{\mathrm{min}}(\bm{p}_{g_{\sigma(j-1)}}, \bm{p}_{g_{\sigma(j)}}) \right\}
\]
ここで、$T_{n^A_i}$とは、$n^A_i$個の数字$1, 2, ..., n^A_i$の置換全体の集合である。
